How Can ChatGPT Support Human Security Testers to Help Mitigate Supply Chain Attacks?

Developers often build software on top of third-party libraries (Libs) to improve productivity, but these libraries may contain vulnerabilities that enable supply chain attacks. Existing tools detect vulnerable dependencies, yet developers often distrust their reports without concrete exploit evidence. Manually crafting such demonstrations is costly, and tool support is lacking. To help developers enhance software security, in this study, we systematically explored the usage of a large language model (LLM) --ChatGPT-4.0--to generate security tests, which unit tests demonstrate how vulnerable library dependencies facilitate the supply chain attacks to given Apps. In our exploration, we defined prompt templates to take in the various vulnerability-relevant information we manually collected, and generated prompts from those templates to query ChatGPT for security test generation. We found that ChatGPT-generated tests demonstrated 24 pieces of evidence or proof of vulnerability for 49 Apps. To assess the consistency of test generation, we also evaluated another five state-of-the-art LLMs. All the models generated security tests for at least 17 cases that successfully demonstrate the vulnerabilities. We filed six reports for the newly revealed vulnerabilities in Apps, and got four Common Vulnerability Entries (CVEs) assigned. Our use of ChatGPT outperformed two state-of-the-art security test generators (TRANSFER and SIEGE), by generating a lot more tests and achieving more attacks.

==> Background.tex <==
\section{Background}
\label{sec:background}
Our background describes the prevalence of vulnerability dependencies used in Java applications; we introduce the current approaches to address vulnerability detection in dependencies, such as Java composition analysis and its limitations. Lastly, we provide background knowledge about \chatgpt.


\subsection{Java Components with Supply-Chain Vulnerabilities}
 The incorporation of vulnerable third-party components in the development of software has increased recently. 
 %rendered numerous benefits, notably efficiency and cost-effectiveness.
%and applications  A report by 
Synoposys~\cite{ahmed2023common} reported that a staggering 97\% of applications now contain at least one open-source component. While many Java applications have been identified with vulnerabilities within their included components or dependencies~\cite{wang2020empirical,kula2018developers}. The depth of this predicament has been expounded by studies from Snyk~\cite{snyk} and Williams et al.~\cite{williams2012unfortunate}, revealing that approximately 67\% of real-world Java projects include dependencies harboring known vulnerabilities. When such compromised libraries are integrated into an application, they can pose severe security threats. Furthermore, these vulnerabilities often persist in projects well beyond their public disclosure and even after patches have become available~\cite{panetta2018gartner}. A research study by Yan \textit{et al.}~\cite{yan2021estimating} uncovered that even bug fix commits were applied to 50 open-source Java projects on GitHub, 939 dependent projects continued to utilize versions of dependencies containing vulnerabilities. This continued use of compromised libraries is attributed primarily to the complexities involved in managing and updating dependencies. 

Moreover, these component vulnerabilities are recorded and traced by many publicly available security databases~\cite{githubadvisories, snyk,booth2013national,hat2007red, vulnerabilities2005common, martin2011cwe}, including the CVE, Snyk, and the National Vulnerability Database (NVD). These repositories catalog publicly disclosed software vulnerabilities, encompassing details about the nature of each vulnerability, and the affected software.  These well-recorded and up-to-date security practices can be back-door attackers to exploit vulnerabilities in the software components. 
%Ladisa and Pashchenko \cite{plate2015impact, ponta2020detection} address the concern, pointed out \textcolor{red}{xx}.
Open Web Application Security Project (OWASP)~\cite{owasp10Vul} reported the use of vulnerable or outdated components has been identified as one of the top 10 web security risks since 2017. Using known vulnerabilities in Java components is a pressing issue in software security. Therefore, exploring approaches to identify and mitigate these vulnerabilities, such as the approach we evaluate in this paper, is of paramount importance for bolstering the security posture of Java-based software applications.

\subsection{Vulnerable Dependencies Analysis and Detection}

\textbf{Dependencies scanner} alters users at an early stage by scanning the project dependency configuration without running the project. Industry tools, such as OWASP Dependency Checker~\cite{dependencychecker}, utilize an extensive security database populated with security entries derived from the NVD and GitHub Security Alerts. These tools function by scanning the application's manifest file, cross-referencing the dependency's version and name information with the corresponding entries in the security database. If a match is found, the scanner generates a security alert, thus enabling the users to update the compromised dependency package accordingly. While Commercial tools~\cite{snykSec, BugTracker}, advanced provides continuous monitoring of the software components, ensuring that security and compliance checks are performed consistently throughout the development lifecycle. 
However, a notable drawback of these tools is their tendency to overestimate vulnerability, which leads to a considerable proportion of false positives within the detection reports.
%To identify the known vulnerability in the client project. Vulnerable dependency analysis aims to alter the user at an early stage by scanning the project dependency configuration~\cite{snykSec, BugTracker, dependencychecker, ohm2020towards, schlumberger2012jarhead, ladisa2022towards}. OWASP Dependency Checker~\cite{dependencychecker} checks the Pom.xml files to identify the known vulnerabilities. It matches the dependency's version and name with the security entries recorded in NVD or GitHub Security Alters. If a Common Platform Enumeration (CPE) is found, the OWASP dependency checker alters uses by generating the report with associated CVE links. Github secu The scanner may overestimate the vulnerability and pose a high false positive in the detection report. 
 
\noindent\textbf{Static analysis} aims to identify third-party dependencies' vulnerabilities without executing or running the code~\cite{ohm2020towards, schlumberger2012jarhead, ladisa2022towards}. Ladisa \textit{et al.}~\cite{ladisa2022towards} employed static analysis on Java bytecode to uncover malicious library packages. Their methodology involved analyzing the entropy of strings within the constant pool and conducting data flow analysis related to any suspicious string to extract sensitive APIs. The identification of malicious packages was achieved by locating these sensitive APIs within the code blocks. Eclipse Steady \cite{ponta2020detection}, on the other hand, combined both static and dynamic analysis to scrutinize software composition. The tool verified the application of fixed patches in CVEs and analyzed vulnerability constructors by contrasting the Abstract Syntax Tree (AST) structures. Furthermore, it traced the call chain of the vulnerability from the client project to the vulnerability target, applying dynamic analysis to validate whether the execution path could indeed reach the vulnerable API."
Even though these approaches built based on call graph analysis provide more accurate detection, it still faces false alarm limitations. 

\noindent\textbf{Dynamic validation} exploits testing technicals to generate the vulnerability triggering input for the client project. Siege~\cite{iannone2021toward} extends the Evosuit~\cite{fraser2011evosuite} to handle vulnerability tests for Java projects. It adopts the genetic algorithm that automatically explores the valid test case, which covers the target vulnerable API's invocation code line. Siege may only sometimes find the optimal solution due to the limitation of genetic algorithms. Besides, the approach has yet to be evaluated on a large scale, and its scalability and performance on real-world software systems are unknown. Transfer~\cite{kang2022test} uses an evolutionary algorithm to generate fitter test cases and seeds the object pool with the carved objects from the library test. It guides client test generation to reproduce the same program state as the library's test case when invoking the vulnerable function. However, Transfer could not produce a test case as the arguments to the vulnerable function lacked inspector functions. It is also limited by its inability to satisfy the irrelevant aspects of the captured triggering conditions.


\subsection{\chatgpt}


%\chatgpt is a chatbot that provides articulate responses in various domains based on requests put by users~\cite{ouyang2022training, cobbe2021training, brown2020language}.  It is a Large language model (LLM) pre-training with massive data. different from the LLM such as Bert~\cite{devlin2018bert}, Transformer-XL \cite{dai2018transformer}, T5\cite{raffel2020exploring}. \chatgpt-3.5 and  \tool \cite{openai2023gpt4, bubeck2023sparks}leverage a combination of supervised and reinforcement learning techniques and use self-attention mechanisms to model the complex relationships between words and their contexts in a sentence. \textcolor{red}{limitation with some 8192 words}
%As shown in figure \ref{fig:gpt}, users provide instructions in 1, \chatgpt will provide the response based on the user's description. The answer includes natural language and code part in 2. since the first instruction is not clear, user may specify more relevant context, \chatgpt is able to provide the feedback based on the context deduction.  
The Generative Pretrained Transformers (GPTs) ~\cite{radford2018improving, gpt2, brown2020language} is a large language model developed based on the transformer architecture \cite{vaswani2017attention}.  They are  designed to generate human-like language in response to given prompts.  The models' complexity has increased over time, with later versions employing a more intricate transformer layer structure and a significantly larger parameter space and utilizing massive volumes of training data.  \chatgpt, corresponding to versions GPT-3.5 ~\cite{ouyang2022training} and beyond, including \tool ~\cite{openai2023gpt4}, takes the functionality a step further. It leverages a combination of supervised learning and reinforcement learning techniques, and utilizes a self-attention mechanism to model relationships between words and their contexts within sentences. \chatgpt is specifically designed for conversational tasks, as depicted in Figure \ref{fig:gpt}. The user provides a prompt, problem descriptions and instructions, in the chatbox \textcolor{red}{\textcircled{1}}, such as \textit{"write a test function in Java language"}, in a natural language format. \tool delivers answers that include natural language descriptions and relevant Java code snippets  in \textcolor{red}{\textcircled{2}}. In detail, it provides an example of a Java function that needs testing and subsequently constructs a corresponding test function within the Junit\cite{junit5} framework. However, the precision of the output depends on the clarity of the user's instruction. If the initial instruction is vague, the user can specify the additional context to guide \tool in  \textcolor{red}{\textcircled{3}}. In such a scenario, \tool can adapt and generate feedback based on the newly provided context.

We selected the latest version \tool for our experiments, considering \tool also offers potential in code generation, debugging, and test generation ~\cite{xie2023chatunitest,yuan2023no,surameery2023use}. By leveraging its ability to generate semantically meaningful text based on input prompts, it can contribute significantly to dynamic vulnerability validation in software dependency. This forms the primary motivation for our research, exploring the effectiveness of \tool in generating security tests to trigger vulnerabilities in software applications with known vulnerabilities. 
\begin{figure}
\centering
\includegraphics[width=.95\linewidth]{figures/ChatGPT.pdf}
\vspace{-.5em}
\caption{\chatgpt overview }\label{fig:gpt}
\vspace{-1.5em}
\end{figure}

==> Future.tex <==
\section{Our Recommendation}


\textbf{Prompt tuning} \tool's result influenced by prompt, users can optimize the prompt by 1) extracting the necessary context of the code, 2) excluding the noise information, and 3) automatically improving the instruction by the response result.  

\noindent \textbf{Multi-shot with feedback}  Our research examines the application of one-round zero-shot prompts with the \tool for vulnerability test generation. Considering the ability of \tool for context deduction\cite{wei2022chain}, the multi-shot\cite{brown2020language} approach allows for an iterative, user-driven feedback loop. For instance, \tool generates a unit test containing a compilation error. Users have the capacity to relay this error information back to the \tool. They can subsequently guide the tool to correct the error, thereby facilitating a step-by-step optimization of the generated answer. This iterative refinement process underscores the utility of multi-shot prompts in improving the overall quality of the work produced by \tool. Our findings suggest that utilizing the multi-shot prompts offers substantial improvements in result precision, effectiveness, and user engagement in the testing process. This, in turn, underscores the necessity of embracing such practices in one's workflow. The use of multi-shot prompts can potentially lead to improved accuracy and effectiveness in the testing generation process. 

\noindent \textbf{fine-tuning for vulnerability test generation}  \tool models are not designed to handle the vulnerability test generation. With tailored training, it's feasible to equip \tool with the capabilities to handle vulnerability generation in a more specialized manner. 1) By supplying a test oracle laden with vulnerability entries to train the model. This will provide a foundation of examples for the model to learn from. 2) Providing code context that is specifically aligned to the user scenario, allows the model to understand the coding environment in which it operates. 3) developers can provide an embedding of the target project to be used as a basis for querying results, thus teaching the model about the specific structures and conventions of the project


==> tmp-table-vulnerability.tex <==
\begin{comment}
\begin{table*}
\footnotesize
\caption{The 33 library vulnerabilities included in our dataset}\label{tab:lib-data}\vspace{-1em}
\begin{tabular}{L{2cm}| L{2cm}| L{3.cm}|L{2.5cm}|L{6.5cm}}
\toprule
\textbf{Vulnerability ID} &\textbf{Library} &\textbf{Affected Library Versions} &\textbf{Vulnerable API(s)} & \textbf{Vulnerability Summary
%\& Description
}\\ \toprule
%\textbf{Vulnerability ID} & \textbf{Vulnerability Description} &\textbf{Library Name} &\textbf{Affected Library Versions}\\ \toprule
CODEC-134 &Apache Commons Codec~\cite{apache-commons-codec} & [, 1.13) &Base64.decodeBase64(...)&%\textbf{
CWE-20: Improper input validation
%:} The APIs would decode some invalid encoded strings into arbitrary values. 
%, enabling security exploitation (e.g., tunneling additional information via seemingly valid Strings).
%&Base32 would decode some invalid Base32 encoded string into arbitrary value 
\\ \hline
CVE-2017-7525 & Jackson Databind~\cite{jackson-databind}& [, 2.6.7.1) [2.7.0, 2.7.9.1) [2.8.0, 2.8.9)&ObjectMapper.readValue(...)&%\textbf{
CWE-502: Deserialization of untrusted data;  CWE-184: Incomplete list of disallowed inputs
%:} 
%The deserialization API would allow an unauthenticated user to perform code execution by sending maliciously crafted inputs.
\\ \hline
CVE-2017-7957 &XStream~\cite{xstream}&[, 1.4.9] &XStream.fromXML(...) &
CWE-20: Improper input validation
%\textbf{Improper Input Validation:} The API mishandles attempts to create an instance of the primitive type ``{\tt void}'' during unmarshalling, leading to a remote application crash.
\\ \hline
CVE-2018-1000613 & Bouncy Castle~\cite{bouncy-castle}&[1.58, 1.60) &XMSSMTPrivateKeyParameters.build(), XMSS.generateKeys()?  & CWE-502: Deserialization of untrusted data;  
CWE-470: Use of externally-controlled input to select classes or code ('unsafe reflection')
%\textbf{Use of Externally-Controlled Input to Select Classes or Code (``Unsafe Reflection''):} The vulnerability in XMSS/XMSS\^{}MT private key deserialization can result in the execution of unexpected code. 
\\ \hline
CVE-2018-1000632 & Dom4j~\cite{dom4j} & [, 2.1.1)& DocumentHelper.createElement() &
CWE-91: XML injection 
% \textbf{XML Injection:} The APIs can result in an attacker tampering with XML documents through XML injection, i.e., by specifying elements or attributes in the XML document.
\\ \hline
CVE-2018-1000873&Jackson Databind
%-modules-java8~\cite{jackson-modules-java8}
&[, 2.9.8)&ObjectMapper.readValue(...)
%DecimalUtils.extractSecondsAndNanos(...)? 
& CWE-20: Improper input validation \\ \hline
CVE-2018-1002200 &Plexus Archiver~\cite{plexus-archiver} &[,3.6.0)& UnArchiver.extract()?& CWE-22: Improper limitation of a pathname to a restricted directory ('path traversal')\\ \hline
CVE-2018-1002201& ZT Zip~\cite{zt-zip}&[, 1.13)&ZipUtil.unpack(...) &CWE-22: Improper limitation of a pathname to a restricted directory ('path traversal') \\ \hline
CVE-2018-11761&Apache Tika~\cite{tika}&[0.1, 1.18]&SAXParser.parse(...)?& CWE-611: 	Improper restriction of XML external entity reference\\ \hline
CVE-2018-12418& Junrar~\cite{junrar} &[,1.0.1)& Archive(...)?&CWE-835: Loop with unreachable exit condition ('infinite loop')\\ \hline
CVE-2018-1274 & Spring Data Commons~\cite{spring-data-commons} & [1.13, 1.13.10], [2.0, 2.0.5] &PropertyPath.from(...)? &CWE-770: Allocation of resources without limits or throttling \\ \hline
CVE-2018-19859& OpenRefine~\cite{OpenRefine}& [, 3.2:beta) &ImportingUtilities.allocateFile(...)? &CWE-22: Improper limitation of a pathname to a restricted directory ('path traversal')\\ \hline
CVE-2018-20227 &RDF4J~\cite{rdf4j}&2.4.2 &ZipUtil.extract(...)? &CWE-22: Improper limitation of a pathname to a restricted directory ('path traversal')\\ \hline
CVE-2019-10093 &Apache Tika&[1.19, 1.21] &StandardParser.parse(...)?& CWE-770: Allocation of resources without limits or throttling \\ \hline
CVE-2019-12402 & Apache Commons Compress~\cite{apache-commons-compress}&[1.15, 1.18]&NioZipEncoding(...)? &CWE-835: Loop with unreachable exit condition ('infinite loop')\\ \hline
CVE-2020-10693 &Hibernate Validator~\cite{hibernate-validator}&[5.0.0, 6.0.20), [6.1.2, 6.1.5), 7.0.0:alpha1&? &CWE-20: Improper input validation\\ \hline
CVE-2020-13956&Apache HttpClient~\cite{httpclient}&[, 4.5.13,), [5.0.0, 5.0.3)&CloseableHttpClient.execute(...)&NVD-CWE-noinfo: Insufficient information\\ \hline
CVE-2020-13973&OWASP JSON Sanitizer~\cite{json-sanitizer}& [,1.2.1)&JsonSanitizer.sanitize(...)?&CWE-79: Improper neutralization of input during web
page generation ('cross-site scripting')\\ \hline
CVE-2020-15250&JUnit4~\cite{junit4}&[4.7, 4.13.1)& TemporaryFolder.newFolder(...)&CWE-732: Incorrect permission assignment for critical resource; CWE-200 Exposure of sensitive information to an unauthorized actor\\ \hline
CVE-2020-26217&XStream&[, 1.4.14)& XStream.fromXML(...)&CWE-78: Improper neutralization of special elements used in an OS command ('OS command injection') \\ \hline
CVE-2020-28052&Bouncy Castle &1.65, 1.66&OpenBSDBCrypt.checkPassword(...)& NVD-CWE-Other: Other\\ \hline
CVE-2020-28491& Jackson Dataformat: CBOR~\cite{jackson-dataformats-binary}&[, 2.11.4), (2.12.0-rc1, 2.12.1) & ?&CWE-770: Allocation of resources without limits or throttling\\ \hline
CVE-2020-5408&Spring Security~\cite{spring-security}&[4.2.0, 4.2.16), [5.0.0, 5.0.16), [5.1.0, 5.1.10), [5.2.0, 5.2.4), [5.3.0, 5.3.2)& BCryptPasswordEncoder.encode(...) &CWE-330: Use of insufficiently random values; CWE-329	Generation of predictable IV with CBC mode\\ \hline
CVE-2021-23899&OWASP JSON Sanitizer&[,1.2.2)&JsonSanitizer.sanitize(...)&CWE-611: Improper restriction of XML external entity
reference \\ \hline
CVE-2021-27568&Json-smart~\cite{json-smart-v1,json-smart-v2}&v1:[, 1.3.2), v2: [, 2.3.1), [2.4, 2.4.1)&JSONParser.parse(...) &CWE-754: 	Improper check for unusual or exceptional conditions\\ \hline
CVE-2021-29425&Apache Commons IO~\cite{apache-commons-io}&[, 2.7)&FileNameUtils.normalize(...)& CWE-22: Improper limitation of a pathname to a restricted directory ('path traversal'); CWE-20: Improper input validation \\ \hline
CVE-2021-30468&Apache CXF~\cite{apache-cxf}&[, 3.3.11), [3.4.0, 3.4.4)&JsonMapObjectReaderWriter.fromJson(...)&CWE-835: Loop with unreachable exit condition ('infinite loop'); CWE-400: Uncontrolled resource consumption\\ \hline
CVE-2022-25845&Fastjson~\cite{fastjson}&[, 1.2.83)&JSON.parseObject(...)&CWE-502	: Deserialization of Untrusted Data\\ \hline
CVE-2022-45688 &hutool-json~\cite{hutool-json} &5.8.10 &XML.toJSONObject(...)&CWE-787: Out-of-bounds Write\\ \hline
CVE-2023-34454&snappy-java~\cite{snappy-java}&[, 1.1.10.1)&Snappy.compress(...)&CWE-190: Integer overflow or wraparound\\ \hline
HTTPCLIENT-1803&Apache HttpClient&[,4.5.3)& &CWE-23: Relative path traversal\\ \hline
TwelveMonkeys-595&TwelveMonkeys~\cite{twelveMonkeys}&[0, 3.6.4)&ImageReader.read(...)&CWE-400: Uncontrolled resource consumption\\ \hline
Zip4j-263&Zip4j~\cite{zip4j}&[0, 2.7.0)&ZipFile(...) & 	
CWE-476: NULL pointer dereference\\ \hline

%&A deserialization flaw in the library, could allow an unauthenticated user to perform code execution by sending the maliciously crafted input to the readValue method of the ObjectMapper

\end{tabular}
\end{table*}
\end{comment}
